SPOT: SE(3) Pose Trajectory Diffusion for Object-Centric Manipulation

We introduce SPOT, an object-centric imitation learning framework. The key idea is to capture each task by an object-centric representation, specifically the SE(3) object pose trajectory relative to the target. This approach decouples embodiment actions from sensory inputs, facilitating learning from various demonstration types, including both action-based and action-less human hand demonstrations, as well as cross-embodiment generalization. Additionally, object pose trajectories inherently capture planning constraints from demonstrations without the need for manually-crafted rules. To guide the robot in executing the task, the object trajectory is used to condition a diffusion policy. We systematically evaluate our method on simulation and real-world tasks. In real-world evaluation, using only eight demonstrations shot on an iPhone, our approach completed all tasks while fully complying with task constraints. Project page: https://nvlabs.github.io/object_centric_diffusion

==> tables/rlbench.tex <==
% \begin{table}[t]
%     \scriptsize
%     \centering
%     \vspace{6mm}
%     \caption{\textbf{Simulation Result on RLBench.} All baselines are multi-task policies conditioned on language description. While RVT2 ran in multi-camera environments, both the 3D Diffuser Actor and our approach utilize only a single camera.}
%     % \vspace{3mm}
%     \resizebox{\columnwidth}{!}{%
%     \begin{tabular}{l|ccccccc}
%     \toprule
%      % & & & & & & & & & & & & & & &\\
%     {\shortstack[c]{Method}} & {\shortstack[c]{Avg. \\ Success}} & {\shortstack[c]{Close \\ Jar}} & {\shortstack[c]{Drag \\ Stick}} & {\shortstack[c]{Insert \\ Peg}} & {\shortstack[c]{Meat off \\ Grill}} & {\shortstack[c]{Place \\ Cups}} & {\shortstack[c]{Place \\ Wine}} \\
    
%     \midrule
    
%     RVT2~\cite{goyal2024rvt} & 76.4 & 98.7 \rpmh 2.3 & 98.7 \rpmh 2.3 & 44.0 \rpmh 6.9 & 96.0 \rpmh 0.0 & 33.3 \rpmh 2.3 & 92.0 \rpmh 4.0  \\
%     3D Diffuser Actor~\cite{ke20243d} & 54.5 & 77.3 \rpmh 0.0 & 92.0 \rpmh 8.0 & 9.3 \rpmh 2.3 & 84.0 \rpmh 0.0 & 4.0 \rpmh 0.0 & 78.7 \rpmh 4.6 \\
%     Ours & 78.9 & 94.7 \rpmh 6.1 & 81.3 \rpmh 2.3 & 72.0 \rpmh 4.0 & 98.7 \rpmh 2.3 & 72.0 \rpmh 0.0 & 100.0 \rpmh 0.0  \\
    
%     \midrule
    
%     {\shortstack[c]{Method}} & {\shortstack[c]{Put in \\ Cupboard}} & {\shortstack[c]{Put in \\ Safe}} & {\shortstack[c]{Screw \\ Bulb}} & {\shortstack[c]{Sort \\ Shape}} & {\shortstack[c]{Stack \\ Blocks}} & {\shortstack[c]{Stack \\ Cups}} & {\shortstack[c]{Turn \\ Tap}} \\
    
%     \midrule
    
%     RVT2~\cite{goyal2024rvt} & 69.3 \rpmh 2.3 & 89.3 \rpmh 8.3 & 86.7 \rpmh 4.6  & 49.3 \rpmh 6.1  & 81.3 \rpmh 6.1 & 60.0 \rpmh 0.0  & 94.7 \rpmh 4.6 \\
%     3D Diffuser Actor~\cite{ke20243d} & 38.7 \rpmh 2.3 & 86.7 \rpmh 2.3 & 38.7 \rpmh 4.6 & 30.7 \rpmh 2.3 & 41.7 \rpmh 7.5 & 30.7 \rpmh 8.3 & 96.0 \rpmh 0.0 \\
%     Ours & 69.3 \rpmh 6.1 & 100.0 \rpmh 0.0 & 48.0 \rpmh 8.0 & 22.7 \rpmh 2.3 & 90.0 \rpmh 2.8 & 78.0 \rpmh 2.8 & 100.0 \rpmh 0.0 \\

%     \bottomrule
    
%     \end{tabular}
%     }
%     \label{tab: rlbench}
%     % \vspace{-5mm}
% \end{table}


\begin{table*}[h]
    % \scriptsize
    \centering
    % \vspace{-10pt}
    % \vspace{-5pt}
    \caption{\textbf{Simulation Results on RLBench.} All methods use a single set of weights to perform multiple tasks, conditioned on language description. 
    % While RVT2 ran in multi-camera environments, both the 3D Diffuser Actor and our approach utilize only a single camera.
    }     \label{tab: rlbench}
    \resizebox{0.8\linewidth}{!}{%
   \begin{tabular}{lc|ccccccc}
\hline
\rowcolor[rgb]{ .706,  .776,  .906}                                & \textbf{Single}                & \textbf{Avg}                   & \textbf{Close}                 & \textbf{Drag}                  & \textbf{Insert}                & \textbf{Meat off}              & \textbf{Place}                 & \textbf{Place} \bigstrut[t]\\
\rowcolor[rgb]{ .706,  .776,  .906} \multicolumn{1}{c}{\textbf{Method}} & \textbf{View}                  & \textbf{Succ.}                 & \textbf{Jar}                  & \textbf{Stick}                & \textbf{ Peg}                  & \textbf{Grill}                 & \textbf{ Cups}                 & \textbf{ Wine} \bigstrut[b]\\
\hline
RVT2~\cite{goyal2024rvt}       & \redxmark                      & 76.4                           & \textbf{98.7 \rpmh 2.3}                 & \textbf{98.7 \rpmh 2.3}                 & 44.0 \rpmh 6.9                 & 96.0 \rpmh 0.0                 & 33.3 \rpmh 2.3                 & 92.0 \rpmh 4.0 \bigstrut[t]\\
3D-DA~\cite{ke20243d}          & \greencheckmark                & 54.5                           & 77.3 \rpmh 0.0                 & 92.0 \rpmh 8.0                 & 9.3 \rpmh 2.3                  & 84.0 \rpmh 0.0                 & 4.0 \rpmh 0.0                  & 78.7 \rpmh 4.6 \\
Ours                           & \greencheckmark                & \textbf{79.4}                           & \textbf{98.7 \rpmh 2.3}                 & 80.0 \rpmh 0.0                 & \textbf{78.7 \rpmh 2.3}                 & \textbf{100.0 \rpmh 0.0}                 & \textbf{62.7 \rpmh 6.1}                 & \textbf{100.0 \rpmh 0.0} \bigstrut[b]\\
\hline
\hline
\rowcolor[rgb]{ .706,  .776,  .906}                                & \textbf{Single}                & \textbf{Put in}                & \textbf{Put in}                & \textbf{Screw}                 & \textbf{Sort}                  & \textbf{Stack }                & \textbf{Stack}                 & \textbf{Turn} \bigstrut[t]\\
\rowcolor[rgb]{ .706,  .776,  .906} \multicolumn{1}{c}{\textbf{Method}} & \textbf{View}                  & \textbf{Cupboard}              & \textbf{ Safe}                 & \textbf{ Bulb}                 & \textbf{ Shape}                & \textbf{Blocks}                & \textbf{ Cups}                 & \textbf{Tap} \bigstrut[b]\\
\hline
RVT2~\cite{goyal2024rvt}       & \redxmark                      & \textbf{69.3 \rpmh 2.3}                 & 89.3 \rpmh 8.3                 & \textbf{86.7 \rpmh 4.6}                 & \textbf{49.3 \rpmh 6.1}                 & 81.3 \rpmh 6.1                 & 60.0 \rpmh 0.0                 & 94.7 \rpmh 4.6 \bigstrut[t]\\
3D-DA~\cite{ke20243d}          & \greencheckmark                & 38.7 \rpmh 2.3                 & 86.7 \rpmh 2.3                 & 38.7 \rpmh 4.6                 & 30.7 \rpmh 2.3                 & 41.7 \rpmh 7.5                 & 30.7 \rpmh 8.3                 & 96.0 \rpmh 0.0 \\
Ours                           & \greencheckmark                & 42.7 \rpmh 4.6                 & \textbf{100.0 \rpmh 0.0}                & 48.0 \rpmh 8.0                 & 32.0 \rpmh 4.0                 & \textbf{94.0 \rpmh 3.4}                 & \textbf{96.0 \rpmh 0.0}                 & \textbf{100.0 \rpmh 0.0} \bigstrut[b]\\
\hline
\end{tabular}%


    }
    %\vspace{-5pt}  % commented for arxiv
\end{table*}
